Automatic Repair of Overflowing Expressions with Abstract Interpretation

We consider the problem of synthesizing provably non-overflowing integer arithmetic expressions or Boolean relations among integer arithmetic expressions. First we use a numerical abstract domain to infer numerical properties among program variables. Then we check if those properties guarantee that a given expression does not overflow. If this is not the case, we synthesize an equivalent, yet not-overflowing expression, or we report that such an expression does not exists. The synthesis of a non-overflowing expression depends on three, orthogonal factors: the input expression (e.g., is it linear, polynomial,... ?), the output expression (e.g., are case splits allowed?), and the underlying numerical abstract domain - the more precise the abstract domain is, the more correct expressions can be synthesized. We consider three common cases: (i) linear expressions with integer coefficients and intervals; (ii) Boolean expressions of linear expressions; and (iii) linear expressions with templates. In the first case we prove there exists a complete and polynomial algorithm to solve the problem. In the second case, we have an incomplete yet polynomial algorithm, whereas in the third we have a complete yet worst-case exponential algorithm.

==> eptcsdata.tex <==
\providecommand{\firstpage}{341}
\providecommand{\publicationstatus}{A. Banerjee, O. Danvy, K.-G. Doh, J. Hatcliff (Eds):\\
David A. Schmidt's 60th Birthday Festschrift\\
EPTCS 129, 2013, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.129.21}{10.4204/EPTCS.129.21}}
\pdfoutput=1

